Transformer Feed-Forward Layers Are Key-Value Memories

Feed-forward layers constitute two-thirds of a transformer model's parameters, yet their role in the network remains under-explored. We show that feed-forward layers in transformer-based language models operate as key-value memories, where each key correlates with textual patterns in the training examples, and each value induces a distribution over the output vocabulary. Our experiments show that the learned patterns are human-interpretable, and that lower layers tend to capture shallow patterns, while upper layers learn more semantic ones. The values complement the keys' input patterns by inducing output distributions that concentrate probability mass on tokens likely to appear immediately after each pattern, particularly in the upper layers. Finally, we demonstrate that the output of a feed-forward layer is a composition of its memories, which is subsequently refined throughout the model's layers via residual connections to produce the final output distribution.

==> obsolete/06_model_output.tex <==


% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.5]{figures/residual_influence_norm_dist_across_layers.pdf}
%     \caption{TBD}
%     \label{figure:residual_influence}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.5]{figures/residual_output_prob_dist_across_layers.pdf}
%     \caption{Probability of the model's output by the residual of each layer.}
%     \label{figure:residual_output_prob}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/residual_predicts_final_output.pdf}
%     \caption{TBD}
%     \label{figure:residual_final_output_preds}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.45]{figures/output_prob_change_ffn_prediction_cases.pdf}
%     \caption{Change in probability of the output token between the output distribution and the residual distribution, for different prediction cases: (A) output = residual $\neq$ ffn, (B)  output = residual = ffn, (C) output $\neq$ residual, residual $\neq$ ffn, ffn $\neq$ output, (D) output = ffn $\neq$ residual. The number of occurrences of each case are shown in parentheses.}
%     \label{figure:ffn_influence_residual}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/prediction_cases.pdf}
%     \caption{Example breakdown by prediction cases: (A) output = residual $\neq$ ffn, (B)  output = residual = ffn, (C) output $\neq$ residual, residual $\neq$ ffn, ffn $\neq$ output, (D) output = ffn $\neq$ residual. There are no cases where output $\neq$ residual = ffn. \omer{we really need to simplify and clarify the notation here.}}
%     \label{figure:prediction_cases}
% \end{figure}




% \section{From FFN Outputs to Model Outputs}
% \label{sec:ffn_residual}

% \omer{The role of the residual? Multi-layer dynamics?}

% \omer{It needs to be stated that now we have proper distributions, since we're no longer detaching the value vector from the coefficient.}

% \omer{I think we need to tell the story the other way around... start from the argmax statistics (this is similar to what we have in the previous section), and then talk about influence as a smoother metric.}

% %Thus far, we have analyzed the FFN sublayers while ignoring their interaction with other components in the network. 
% %To analyze how the FFN's output is converted into the final model prediction, the network residual must be considered.
% % However, an important mechanism in Transformer that could influence the FFN's functionality is the addition of the residual, which propagates information from previous layers. 
% As a case study, we characterize how the last FFN layer is aggregated with other outputs to produce the model's output. The output is produced by summing the layer's output with a residual connection $\mathbf{r}$, and taking the softmax of dot-products of each element in the embedding matrix $E$, i.e.,
% $$ \mathbf{y} = \text{Softmax}((FFN(\mathbf{h}) + \mathbf{r})\cdot E) $$ 
% % In \S\ref{sec:w2_as_values}, we have showed that columns in $B$ in the last layer are correlated with output embeddings. 
% % In order to understand how the final prediction of the model is made, 

% where $\mathbf{r}$ is equal to the FFN layer's input.\roei{maybe just use the same notation $\mathbf{x}$?}

% %In this section, we conduct experiments to understand the role of the FFN's output in the model's prediction. 
% %We measuring the influence of FFN's output in the final prediction in comparison to the residual, and analyze the how the FFN's output changes the residual's prediction.


% \paragraph{$\mathbf{r}$ vs. $FFN(\mathbf{h})$.}
% We aim to determine which of the two elements is dominant in this computation. To this end, we zero out each element and perform the output computation again for the examples from Section~\ref{subsec:ffn_pattern_aggregation}. We define the \textit{influence} of an element (either $\mathbf{r}$ or $FFN(\mathbf{h})$) as the distance between the output probability before and after setting it to zero. Distribution distance is computed via KL divergence $KL(\mathbf{p}||\mathbf{q}) = \sum_{i=1}^{|V|} p_i \cdot \log\Big(\frac{p_i}{q_i}\Big)$, and normalized the two influence scores by their sum to get a relative score.
% %distance between the output distribution and the distribution over the vocabulary when zeroing-out $\mathbf{r}$.%Let $\mathbf{q} = \mathbf{p}_{FFN} = \text{Softmax}(FFN(\mathbf{h})\cdot E)$ be the distribution over the vocabulary induced by the FFN (residual is zeroed-out), we define the \textit{influence} of $\mathbf{r}$ for an input hidden state $\mathbf{h}$ as:
% %$$ \mathcal{I}_{\mathbf{r}}({\mathbf{h}}) = KL(\mathbf{y}||\mathbf{q}) = \sum_{i=1}^{|V|} y_i \cdot \log\Big(\frac{y_i}{q_i}\Big)$$
% %Similarly, we define the influence of the FFN as $\mathcal{I}_{FFN}({\mathbf{h}}) = KL(\mathbf{y}||\mathbf{p})$, where $\mathbf{p} = \text{Softmax}(\mathbf{r}\cdot E)$.

% Figure~\ref{figure:residual_influence} depicts the relative influence of the residual across the network layers.
% The minimal influence of $\mathbf{r}$ is 75\%, indicating that the distribution chosen via aggregating all lower layers of the model is more dominant than the distribution induced by the single last layer.
% %Thus, the network's residual $\mathbf{r}$ largely determines the output, yet an FFN layer's output ``refines'' it.


% \paragraph{A layer's output refines the prediction.}

% \omer{This experiment is super-hard to follow, and I think we should (a) simplify it, and provide just the argmax statistics, (b) do it for every layer, and show how the residual becomes more static.}

% \omer{I would also rename the classes to something informative, like: ``Same'', ``Residual'', ``FFN'', ``Other''.}

% We now analyze the maximal probability assigned to an output token (the model's \textit{prediction confidence}), in (1) the models' output distribution, (2) the distribution induced by the FFN layer's output (the residual zeroed out), and (3) the distribution induced by the residual (the FFN layer output zeroed out).
% %With a minimum influence of 75\%, it is apparent that the residual, which propagates information from previous layers, highly influences the output of each layer. 
% %Correspondingly, the maximal influence of the FFN sublayer is $<25\%$.
% %
% %\paragraph{The FFN tunes the residual predictions}
% %To assess the FFN's influence on the residual in construction of the final output, we measure the change in probability of the output token before and after aggregating the FFN's with the residual, i.e. $\mathbf{y}(y) - \mathbf{p}(y)$ where $y = \arg\max(\mathbf{y})$
% Figure~\ref{figure:ffn_influence_residual} describes the change in the output probability when the residual and FFN predictions match and do not match the final output.
% For most of the examples (cases A and B), the residual prediction matches the final output. This is expected given the high influence of the residual. 
% Usually (case A), the FFN's output is different from this of the residual, and there is no clear trend in the output probability.
% However, when the FFN matches the residual prediction (case B), it boosts the output probability, often by more than 10\%.
% Lastly, when adding the FFN modifies the prediction (cases C and D), there is almost always a small boost in probability, which becomes substantial (>20\%) when the FFN prediction matches the final output.
% It seems as if the FFN layer's output, when added to the network's residual, only slightly changes the output distribution yet significantly increases the model's confidence in its prediction.

% %These results show how the FFN ``fine-tunes'' the residual predictions, usually increasing the probability of the output token.

% \begin{table}[t]
%     \centering
%     \footnotesize
%     \begin{tabular}{c|c}
%          &  probability \\ \hline
%          A & 40.5 $\pm$ 25.8 \\
%          B & 70.8 $\pm$ 25.4 \\
%          C & 17.8 $\pm$ 14.5 \\
%          D & 34.7 $\pm$ 1.0 
%     \end{tabular}
%     \caption{Residual prediction probability.}
%     \label{table:residual_confidende}
% \end{table}
 
% We further analyze the cases when the FFN modifies the residual output and find that in most cases (54 examples), the modification is dramatic (e.g. \nl{Standards} $\rightarrow$ \nl{Land}) and in the rest of the cases (17 examples), the FFN's output shifts the residual prediction to a close token (e.g. \nl{Byzantines} $\rightarrow$ \nl{Byzantine} and \nl{two} $\rightarrow$ \nl{five}).

% Table~\ref{table:residual_confidende} shows the confidence of the distribution induced by the residual in each case. 
% High confidence is assigned when predictions match the output ones (cases A and B), especially when the FFN also supports the same prediction (case B). Conversely (cases C and D), when the residual does not match the output, its prediction is less confident. This is expected since, to begin with, the top token in less confident residual distributions is more likely to be altered when adding the FFN output.


